Feedback effect on the observable properties of $z>6$ AGN

Active galactic nuclei (AGN) feedback has a major impact onto the supermassive black-hole (SMBH) growth, the properties of the host galaxies, and their cosmic evolution. We investigate the effects of different kinetic feedback prescriptions on the observable properties of AGN and their host galaxies at $z>6$ in a suite of zoom-in cosmological simulations. We find that kinetic feedback decreases the column density of the interstellar medium (ISM) in the host galaxy by up to a factor of $\approx10$, especially when the SMBHs reach high accretion rates ($\approx10-30\,\mathrm{M_\odot\,yr^{-1}}$). In particular, kinetic feedback is required to extend the ISM size to $>1$ kpc and match the observed sizes of the gas reservoirs in $z>6$ AGN host galaxies. Moreover, it produces unobscured lines of sight along which the AGN can be detected in the rest-frame UV band with magnitudes consistent with observed values of $z>6$ AGN. The assumed geometry of the outflow plays an important role in shaping the observed properties of high-redshift AGN. We find that a biconical geometry is favored over a spherical one to reproduce the observed properties, but it overestimates the number of multiple AGN systems detectable in X-ray observations. This result suggests that simplistic BH seeding recipes widely employed in cosmological simulations produce too many X-ray detectable multiple AGN at $z=6-7$, thus soliciting the adoption of more physically motivated seeding prescriptions.

==> Fabio Vito (Column densities)/include_tex/additional_def.tex <==

% element astro-like
\def\HI{\hbox{H~$\scriptstyle\rm I $~}}
\def\HII{\hbox{H~$\scriptstyle\rm II $~}}
\def\HeI{\hbox{He~$\scriptstyle\rm I $~}}
\def\HeII{\hbox{He~$\scriptstyle\rm II $~}}
\def\HeIII{\hbox{He~$\scriptstyle\rm III $~}}
%
%\def\CIIion{\hbox{C~$\scriptstyle\rm II $}}
%\def\OIion{\hbox{O~$\scriptstyle\rm I $}}
%\def\OIIIion{\hbox{O~$\scriptstyle\rm III $}}
%\def\NIIion{\hbox{O~$\scriptstyle\rm II $}}
%
\def\CIIion{${\rm C}^{+}$}
\def\OIIIion{${\rm O}^{++}$}
\def\NIIion{${\rm N}^{+}$}

% FIR emission lines
\def\CII{\hbox{[C~$\scriptstyle\rm II $]}}
\def\OI{\hbox{[O~$\scriptstyle\rm I $]}} 
\def\OIII{\hbox{[O~$\scriptstyle\rm III $]}} 
\def\NII{\hbox{[N~$\scriptstyle\rm II $]}}

% absorption lines
\def\MGII{\hbox{Mg~$\scriptstyle\rm II $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV $}}
\def\SiI{\hbox{Si~$\scriptstyle\rm I $}}
\def\SII{\hbox{Si~$\scriptstyle\rm II $}} 
\def\NIIa{\hbox{N~$\scriptstyle\rm IIa $}} 

\def\red{\color{red}}
\def\green{\color{green}}
\def\cyan{\color{cyan}}

% mnras style for code names
\newcommand\code[1]{\textsc{\MakeLowercase{#1}}}
\newcommand{\quotes}[1]{``#1''}
\newcommand{\quotesing}[1]{`#1'}

% cosmo
\def\vir{\rm vir}
\def\halo{\rm h}
\def\cent{\rm c}
\def\rvir{r_{\vir}}
\def\zlos{\langle Z\rangle}
%
\def\diinu{\Delta I_{\nu}\slash I_{\nu}}
\def\diiDnu{\Delta I\slash I}
\def\mujb{\mu {\rm Jy}/{\rm beam}}

% math
\def\gt{$>$}

% chemistry
\def\nh2{n_{\rm H2}}
\def\fh2{f_{\rm H2}}
\def\fhp{f_{\rm H+}}
\def\Hp{${\rm H}^{+}$}
\def\dust{\mathcal{D}}
\def\mp{m_{\rm p}}

% units
\def\arcsec{^{\prime\prime}}
\def\angstrom{\textrm{A\kern -1.3ex\raisebox{0.6ex}{$^\circ$}}}
\def\myr{\rm Myr}
\def\mum{\mu{\rm m}}
% solar stuff
\def\msun{{\rm M}_{\odot}}
\def\zsun{{\rm Z}_{\odot}}
\def\lsun{{\rm L}_{\odot}}
\def\dsun{\dust_{\odot}}
%
\def\cc{{\rm cm}^{-3}}
\def\colcm{{\rm cm}^{-2}}
%
\def\msunyr{\msun\,{\rm yr}^{-1}}
\def\surfd{\msun\,{\rm kpc}^{-2}}
\def\surfsfr{\msun\,{\rm yr}^{-1}\,{\rm kpc}^{-2}}
\def\surfdpc{\msun\,{\rm pc}^{-2}}
\def\surfl{\lsun\,{\rm kpc}^{-2}}
%
\def\kpc{{\rm kpc}}
\def\SFR{{\rm SFR}}

%lum and ions
\def\SCII{\Sigma_{\rm [CII]}}
\def\SOIII{\Sigma_{\rm [OIII]}}
\def\SNII{\Sigma_{\rm [NII]}}
\def\SigmaCII{\Sigma_{\rm C+}}
\def\SigmaOIII{\Sigma_{\rm O++}}
\def\SigmaNII{\Sigma_{\rm N+}}
% additional convenience stuff
\def\sigmasfr{\dot{\Sigma}_{\star}}

% names shortcuts
\def\althaea{Alth{\ae}a}
\def\highz{$\mbox{high-}z$~}
\def\noAGN{\emph{noAGN} }
\def\AGNsphere{\emph{AGNsphere} }
\def\AGNcone{\emph{AGNcone} }
\def\amin{a_{\rm min}}

==> Fabio Vito (Column densities)/include_tex/colors.tex <==

% workaround for colors starging with f
\makeatletter
\def\@hex@@Hex#1%
 {\if a#1A\else \if b#1B\else \if c#1C\else \if d#1D\else
  \if e#1E\else \if f#1F\else #1\fi\fi\fi\fi\fi\fi \@hex@Hex}
\makeatother

\definecolor{apcolor}{HTML}{008000}
\definecolor{cbcolor}{HTML}{ff0f00}
\definecolor{afcolor}{HTML}{b3443c}
\definecolor{ddcolor}{HTML}{077a2f}
\definecolor{fdcolor}{HTML}{0e3466}
\definecolor{sgcolor}{HTML}{b3003b}
\definecolor{fvcolor}{HTML}{8900bf}

\newcommand{\AP}[1]{({\bf \color{apcolor} AP: #1})}
\newcommand{\AF}[1]{({\bf \color{afcolor} AF: #1})}
\newcommand{\dd}[1]{({\bf \color{ddcolor} DD: #1})}
\newcommand{\CB}[1]{({\bf \color{cbcolor} CB: #1})}
\newcommand{\FD}[1]{({\bf \color{fdcolor} FD: #1})}
\newcommand{\SG}[1]{({\bf \color{sgcolor} SG: #1})}
\newcommand{\FV}[1]{({\bf \color{fvcolor} FV: #1})}


==> Fabio Vito (Column densities)/include_tex/definizioni.tex <==
\def\be{\begin{equation}} 
\def\ee{\end{equation}} 
\def\ba{\begin{eqnarray}} 
\def\ea{\end{eqnarray}} 
\def\erfc{\rm {erfc}} 
\def\bbf{\bf} 
\def\mpc{\,{\rm {Mpc}}} 
\def\mpch{\,h^{-1}{\rm {Mpc}}} 
\def\kms{\,{\rm {km\, s^{-1}}}} 
\def\cc{\,{\rm {cm^{-3}}}} 
\def\msun{{\Msun}} 
\def\vcir{{v_c}}  
\def\dt{{\Delta t}}  
\def\Gyr{{\,\rm Gyr}} 
\def\etal{{\it et al.~}}  
\def\Hm{${\rm {H^-}}\,\,$}  
%\def\HH{${\rm {H_2}}\,\,$}
\def\HH{${\rm {H_2}}$}
\def\HHp{${\rm {H_2^+}}\,\,$} 
\def\sngg{SN$_{\gamma\gamma}$~}  
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{\esc}} 
\def\HI{\hbox{H~$\scriptstyle\rm I\ $}} 
\def\HII{\hbox{H~$\scriptstyle\rm II\ $}} 
\def\HeI{\hbox{He~$\scriptstyle\rm I\ $}} 
\def\HeII{\hbox{He~$\scriptstyle\rm II\ $}} 
\def\HeIII{\hbox{He~$\scriptstyle\rm III\ $}} 
\def\CIV{\hbox{C~$\scriptstyle\rm IV\ $}} 
\def\SIV{\hbox{Si~$\scriptstyle\rm IV\ $}} 
\def\OVI{\hbox{O~$\scriptstyle\rm VI\ $}} \def\nHI{{\rm HI}} 
\def\nCIV{{\rm CIV}} \def\nOVI{{\rm OVI}} \def\nH{{\rm H}} 
\def\nHII{{\rm HII}} \def\nHe{{\rm He}} \def\nHeI{{\rm HeI}} 
\def\nHeII{{\rm HeII}} \def\nHeIII{{\rm HeIII}} \def\erg{{\rm erg}} 
\def\sr{{\rm sr}} \def\hz{{\rm Hz}} \def\cm{${\rm cm}$} 
\def\nhi{{N_{\rm HI}}} \def\sec{{\rm s}} 
\def\sigmaba{\sigma_8/usr/local/lib/tex/inputs/latex/styles} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} \def\gtsima{$\; \buildrel > \over 
\sim \;$} \def\ltsima{$\; \buildrel < \over \sim \;$} \def\prosima{$\; 
\buildrel \propto \over \sim \;$} \def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} \def\la{\lsim} \def\ga{\gsim} 
\def\ie{{\frenchspacing\it i.e. }} \def\eg{{\frenchspacing\it e.g. }} 
 \def\gtsima{$\; \buildrel > \over \sim \;$} 
\def\ltsima{$\; \buildrel < \over \sim \;$} 
\def\gsim{\lower.5ex\hbox{\gtsima}} 
\def\lsim{\lower.5ex\hbox{\ltsima}} 
\def\simgt{\lower.5ex\hbox{\gtsima}} 
\def\simlt{\lower.5ex\hbox{\ltsima}} 
\def\simpr{\lower.5ex\hbox{\prosima}} 
\def\la{\lsim} 
\def\ga{\gsim} 
\def\de{{\rm d}}
\def\del{\partial}
\def\zcr{Z_{\rm cr}} 
\def\ekin{\mbox{\cal E}_{\rm kin}} 
\def\ekin{{\cal E}_{\rm kin}} 
\def\fgg{f_{\gamma\gamma}} 
\def\fesc{f_{esc}} 
\def\Lya{Ly$\alpha$~} 
\def\sngg{SN-e$^{\pm}$~} 
\def\snggo{SN-e$^{\pm}$} 
\def\msun{\,{\rm \Msun}} 
\def\ie{{\frenchspacing\it i.e., }} 
\def\eg{{\frenchspacing\it e.g., }} 
\def\E3{{\cal E}_{\rm g}^{III}} 
\def\Eunit{\times10^{51} {\rm erg} \, \Msun^{-1}} 
\def\sEunit{10^{51} {\rm erg} \, \Msun^{-1}} 
\def\ozs{\Omega_Z^{sfh}} 
\def\ozo{\Omega_Z^{obs}} 
\def\Onot{\Omega_0} 
\def\Msun{\rm M_\odot}
\def\Zsun{\rm Z_\odot}
\def\rvir{r_{vir}}
\def\rvir{r_{vir}}
\def\vvir{v_{vir}} 
\def\mvir{M_{vir}} 
\def\Tvir{T_{vir}} 
\def\r12{r_{1/2}} 
\def\x12{x_{1/2}} 
\def\v12{v_{1/2}}
\def\ftd{F_{T,D}}
\def\Msf{M_{sf}}


==> Fabio Vito (Column densities)/include_tex/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother


==> Fabio Vito (Column densities)/include_tex/journals.tex <==
\def\amp{\&}
\def\nat{Nature}
\def\na{New Astronomy}
\def\pra{Phys. Rev. A}
\def\prb{Phys. Rev. B}
\def\prc{Phys. Rev. B}
\def\prd{Phys. Rev. D}
\def\mnras{MNRAS}
\def\apj{ApJ}
\def\apjl{ApJL}
\def\apjs{ApJS}
\def\aap{A\&A}
\def\aaps{A\&A Supp.}
\def\aapr{A\&A Rev.}
\def\araa{ARA\&A}
\def\aj{AJ}
\def\qjras{QJRAS}
\def\physrep{Phys. Rep.}
\def\apss{Ap\&SS}               % Astrophysics and Space Science
\def\planss{P\&SS}              % Planetary and Space Science
\def\pasa{Publ. Astr. Soc. Australia}
\def\pasp{Publ. Astr. Soc. Pac.}
\def\jcp{J. Chem. Phys.}
\def\pasj{Pub. Astron. Soc. Japan}
\def\ssr{Space Science Reviews}
\def\grl{Geophysical Research Letters}
\def\jgr{Journal of Geophysical Research}
\def\nar{New Astronomy Reviews}
\def\jcap{JCAP}
\def\fcp{Fundamentals of Cosmic Physics}



==> Fabio Vito (Column densities)/include_tex/pacchetti.tex <==
\usepackage[english]{babel}
\usepackage{amsmath,amssymb}

\usepackage{graphicx}

\usepackage[normalem]{ulem}

\usepackage{verbatim}
\usepackage{color}
\usepackage{multirow}
\usepackage{mathtools}
\usepackage{epstopdf}

\usepackage{url}
\usepackage{xcolor}

\usepackage{gensymb}

\usepackage[usestackEOL]{stackengine}
\usepackage{xspace}


==> include_tex/hyperlink_hack.tex <==

%-----------------------------------------
% avoids the 
%   \pdfendlink ended up in different nesting level than \pdfstartlink.\AtBegShi@Output ...ipout \box \AtBeginShipoutBox
% error
%-----------------------------------------
%
% see https://tex.stackexchange.com/questions/249579/pdfendlink-ended-up-in-different-nesting-level-than-pdfstartlink-error-with

% different workaround
%\AtBeginShipout{%
%  \ifnum\value{page}>1 %
%    \typeout{* Additional boxing of page `\thepage'}%
%    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
%  \fi
%}

\usepackage{etoolbox}
\makeatletter
\newcount\c@additionalboxlevel
\setcounter{additionalboxlevel}{0}
\newcount\c@maxboxlevel
\setcounter{maxboxlevel}{1}
\patchcmd\@combinedblfloats{\box\@outputbox}{%
  \stepcounter{additionalboxlevel}%
  \box\@outputbox
}{}{\errmessage{\noexpand\@combinedblfloats could not be patched}}

\AtBeginShipout{%
  \ifnum\value{additionalboxlevel}>\value{maxboxlevel}%
    \typeout{Warning: maxboxlevel might be too small, increase to %
      \the\value{additionalboxlevel}%
    }%
  \fi 
  \@whilenum\value{additionalboxlevel}<\value{maxboxlevel}\do{%
    \typeout{* Additional boxing of page `\thepage'}%
    \setbox\AtBeginShipoutBox=\hbox{\copy\AtBeginShipoutBox}%
    \stepcounter{additionalboxlevel}%
  }%
  \setcounter{additionalboxlevel}{0}%
}
\makeatother

